Learning production functions for supply chains with graph neural networks

The global economy relies on the flow of goods over supply chain networks, with nodes as firms and edges as transactions between firms. While we may observe these external transactions, they are governed by unseen production functions, which determine how firms internally transform the input products they receive into output products that they sell. In this setting, it can be extremely valuable to infer these production functions, to improve supply chain visibility and to forecast future transactions more accurately. However, existing graph neural networks (GNNs) cannot capture these hidden relationships between nodes' inputs and outputs. Here, we introduce a new class of models for this setting by combining temporal GNNs with a novel inventory module, which learns production functions via attention weights and a special loss function. We evaluate our models extensively on real supply chains data and data generated from our new open-source simulator, SupplySim. Our models successfully infer production functions, outperforming the strongest baseline by 6%-50% (across datasets), and forecast future transactions, outperforming the strongest baseline by 11%-62%

==> reproducibility.tex <==
\section*{Reproducibility Checklist}
Unless specified otherwise, please answer “yes” to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled “Reproducibility Checklist” at the end of the technical appendix.

This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced: \yes
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results: \yes
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper: \yes
\end{itemize}

\noindent Does this paper make theoretical contributions? \no

\noindent Does this paper rely on one or more datasets? \yes 
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets: \yes
    \item All novel datasets introduced in this paper are included in a data appendix: \partialcheck. Synthetic datasets are provided on GitHub (\github). Real supply chains datasets are proprietary and cannot be shared.
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \partialcheck. Our GitHub will be made public, including our synthetic datas and simulator \texttt{SupplySim}.
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. \NA
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. \NA
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. \yes. Our experiments require large-scale, transaction-level supply chains data, which (to the best of our knowledge) is not available publicly, so we turned to the proprietary data from TradeSparq.
    We describe this data in detail in Section~\ref{sec:hitachi-data} and Appendix~\ref{sec:hitachi-data-details}. 
    Also, to promote future research transparency, we have built a simulator that can generate realistic supply chains data, so that future researchers can work on public datasets. 
\end{itemize}

\noindent Does this paper include computational experiments? \yes
\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix: \yes. On GitHub.
    \item All source code required for conducting and analyzing the experiments is included in a code appendix: \yes. On GitHub.
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes: \yes
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from: \yes
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results: \yes,
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks: \yes
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics: \yes
    \item This paper states the number of algorithm runs used to compute each reported result: \yes 
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information: \yes 
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank): \yes 
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments: \yes. See Table~\ref{tab:hyperparameters}.
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting: \yes
\end{itemize}


